Learning Efficient Surrogate Dynamic Models with Graph Spline Networks

While complex simulations of physical systems have been widely used in engineering and scientific computing, lowering their often prohibitive computational requirements has only recently been tackled by deep learning approaches. In this paper, we present GraphSplineNets, a novel deep-learning method to speed up the forecasting of physical systems by reducing the grid size and number of iteration steps of deep surrogate models. Our method uses two differentiable orthogonal spline collocation methods to efficiently predict response at any location in time and space. Additionally, we introduce an adaptive collocation strategy in space to prioritize sampling from the most important regions. GraphSplineNets improve the accuracy-speedup tradeoff in forecasting various dynamical systems with increasing complexity, including the heat equation, damped wave propagation, Navier-Stokes equations, and real-world ocean currents in both regular and irregular domains.

==> figures/ablations.tex <==
\begin{figure*}[ht!]
    \centering
    % \vspace{-5mm}
    \includegraphics[width=.85\textwidth]{figures/ablations.pdf}
    \vspace{-2mm}
    \caption{Ablation studies for the \ourmodel{} architecture. (a) Pareto front of different interpolation algorithms and collocation points in terms of accuracy and speed: \baseline{s}+OSC shows the most efficient performance. (b) MSE of $5$-second rollout predictions of \baseline{}-based models with different numbers of sample points, comparing with the pure \baseline{} model at higher-resolution input of $(64\times 64)$. (c) MSE comparison between the \baseline{} and the \baseline{+OSC} demonstrates the latter contains long rollout errors better.}
    \label{fig:ablations}
    % \vspace{-2mm}
\end{figure*}


    % \caption{\footnotesize Pareto front of different interpolation and collocation points in terms of accuracy and speed with \baseline{s} exhibits the advantages of the OSC method.}
    % \caption{\footnotesize MSE of $5$ second rollout prediction of MPNN based models with differnet number of sample points, comparing with the pure MPNN model taking all $(64\times 64)$ points as input.}
    % \caption{\footnotesize MSE comparision between the \baseline{} and the \baseline{+OSC} with different rollout steps. \baseline{+OSC} contains long rollout errors better than standard \baseline{}.}
    
% \begin{figure*}[h]
%     \centering
%     % \vspace{-5mm}
%     \begin{subfigure}[t]{0.28\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/pareto_front_accuracy_speed.pdf}
%         % \caption{DevFormer and CSE component analysis}
%         \vspace{-7mm}
%         \caption{}
%         \label{fig:ablation_a}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[t]{0.28\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/mse_collocation_points.pdf}
%         \vspace{-7mm}
%         \caption{}
%         \label{fig:ablation_b}
%     \end{subfigure}
%     \quad
%     \begin{subfigure}[t]{0.28\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/error_propagation_rollout.pdf}
%         % \caption{\textcolor{blue}{Performance comparison with number of decap variation on HBM}}
%         \vspace{-7mm}
%         \caption{}
%         \label{fig:ablation_c}
%     \end{subfigure}
%     \vspace{-3mm}
%     \caption{Ablation studies for the \ourmodel{} architecture. (a) Pareto front of different interpolation and collocation points in terms of accuracy and speed: \baseline{s}+OSC shows the most efficient performance. (b) MSE of $5$-second rollout predictions of MPNN-based models with different numbers of sample points, comparing with the pure \baseline{} model at higher-resolution input of $(64\times 64)$. (c) MSE comparison between the \baseline{} and the \baseline{+OSC} demonstrates the latter contains long rollout errors better. \fede{update figure handles in main text!!}}
%     \label{fig:ablations}
%     % \vspace{-6mm}
% \end{figure*}

==> sections/back_matter/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> tables/separated.tex <==

\begin{table}[]
    \scriptsize
    \centering
    \begin{tabular*}{\textwidth}{l | ccccc | cc} 
        \toprule
        \textbf{Model} & \makecell{$\mathbf{1}$\textbf{(s) MSE} \\$\times10^{-3}$} & \makecell{$\mathbf{2}$\textbf{(s) MSE}\\$\times10^{-3}$} & \makecell{$\mathbf{3}$\textbf{(s) MSE} \\$\times10^{-3}$} & \makecell{$\mathbf{4}$\textbf{(s) MSE}\\$\times10^{-3}$} & \makecell{$\mathbf{5}$\textbf{(s) MSE}\\$\times10^{-3}$} & \makecell{Run time for\\$5(s)$ prediction} & \makecell{Rollout steps for \\ $5(s)$ prediction}  \\
        \midrule
        GCN               & $0.5199$ & $0.8876$ & $2.5899$ & $4.1223$ & $6.8703$ & $3.2657$ & $50$ \\ 
        GCN(MLP)          & $0.4846$ & $0.6710$ & $2.0455$ & $3.8761$ & $5.0224$ & $3.0231$ & $50$ \\ 
        GEN               & $\mathbf{0.2322}$ & $0.5291$ & $1.5331$ & $2.0766$ & $2.9223$ & $6.8787$ & $50$ \\ 
        \midrule                                                                                  
        \baseline{}              & $0.3731$ & $0.6020$ & $1.8581$ & $2.6792$ & $3.0880$ & $6.9887$ & $50$ \\ 
        \baseline+OSC(Post)     & $0.3820$ & $0.6891$ & $1.2808$ & $1.4881$ & $1.6793$ & $1.5242$ & $12$  \\ 
        \baselineOSC           & $0.3802$ & $0.5682$ & $0.9244$ & $1.0199$ & $1.1402$ & $\mathbf{1.3822}$ & $12$  \\
        \baseline +OSC+Adaptive  & $0.2678$ & $\mathbf{0.4611}$ & $\mathbf{0.8721}$ & $\mathbf{0.9622}$ & $\mathbf{1.0728}$ & $1.4126$ & $12$  \\ 
        \bottomrule
    \end{tabular*}
    \caption{\small Mean square error on the heat equation dataset. Smaller is better ($\downarrow$). \fede{Merge tables; stds; reduce significant digits}}
    \label{tab:heat-equation-quantitative-analysis}
\end{table}


\begin{table}[]
    \scriptsize
    \centering
    \begin{tabular*}{\textwidth}{l | ccccc | cc} 
        \toprule
        \textbf{Model} & \makecell{$\mathbf{2}$\textbf{(s) MSE} \\$\times10^{-1}$} & \makecell{$\mathbf{4}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{$\mathbf{6}$\textbf{(s) MSE} \\$\times10^{-1}$} & \makecell{$\mathbf{8}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{$\mathbf{10}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{Run time for\\$10(s)$ prediction} & \makecell{Rollout steps for\\$10(s)$ prediction}  \\
        \midrule
        GCN               & $1.4728$ & $2.0133$ & $2.8132$ & $3.5150$ & $4.2455$ & $0.9131$ & $10$ \\ 
        GCN(MLP)          & $1.1222$ & $1.7580$ & $2.4543$ & $2.9443$ & $3.9101$  & $0.8815$ & $10$ \\ 
        GEN               & $0.4217$ & $0.9871$ & $1.6332$ & $2.3848$ & $3.4500$  & $1.0112$ & $10$ \\ 
        \midrule                                                                                   
        \baseline{}              & $0.6623$ & $1.1349$ & $1.6494$ & $2.5778$ & $3.6591$  & $1.2001$ & $10$ \\ 
        \baseline +OSC(Post)     & $0.7204$ & $1.2001$ & $1.6625$ & $1.9825$ & $2.5848$  & $0.5151$ & $5$  \\ 
        \baseline +OSC           & $0.7025$ & $1.0121$ & $1.4448$ & $1.7201$ & $2.2131$  & $\mathbf{0.4778}$ & $5$  \\
        \baseline +OSC+Adaptive  & $\mathbf{0.5433}$ & $\mathbf{0.8071}$ & $\mathbf{1.2322}$ & $\mathbf{1.5005}$ & $\mathbf{2.0214}$  & $0.4927$ & $5$  \\ 
        \bottomrule
    \end{tabular*}
    \caption{\small Mean square error on the wave dataset. Smaller is better ($\downarrow$). \fede{Merge tables; stds; reduce significant digits}}
    \label{tab:wave-quantitative-analysis}
\end{table}

\begin{table}[]
    \scriptsize
    \centering
    \begin{tabular*}{\textwidth}{l | ccccc | cc} 
        \toprule
        \textbf{Model} & \makecell{$\mathbf{2}$\textbf{(s) MSE} \\$\times10^{-1}$} & \makecell{$\mathbf{4}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{$\mathbf{6}$\textbf{(s) MSE} \\$\times10^{-1}$} & \makecell{$\mathbf{8}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{$\mathbf{10}$\textbf{(s) MSE}\\$\times10^{-1}$} & \makecell{Run time for\\$10(s)$ prediction} & \makecell{Rollout steps for\\$10(s)$ prediction}  \\
        \midrule
        GCN               & $1.6199$ & $3.2551$ & $5.1243$ & $7.7720$ & $10.529$ & $0.9520$ & $10$ \\ 
        GCN(MLP)          & $1.4171$ & $2.8552$ & $4.8842$ & $6.0112$ & $9.9021$  & $0.8278$ & $10$ \\ 
        GEN               & $\mathbf{0.7120}$ & $\mathbf{1.4011}$ & $2.9887$ & $4.3442$ & $6.4922$  & $1.1335$ & $10$ \\ 
        \midrule                                                                                   
        \baseline{}              & $0.7957$ & $1.6001$ & $3.2731$ & $5.2782$ & $7.8220$  & $1.3872$ & $10$ \\ 
        \baseline +OSC(Post)     & $0.8120$ & $1.6990$ & $2.5757$ & $3.8810$ & $4.9889$  & $0.4538$ & $5$  \\ 
        \baseline +OSC           & $0.7833$ & $1.5988$ & $2.4822$ & $3.4127$ & $4.6010$  & $\mathbf{0.3991}$ & $5$  \\
        \baseline +OSC+Adaptive  & $0.7482$ & $1.4181$ & $\mathbf{2.2880}$ & $\mathbf{3.3622}$ & $\mathbf{4.5112}$  & $0.4241$ & $5$  \\ 
        \bottomrule
    \end{tabular*}
    \caption{\small Mean square error on the Navier-Stokes equation dataset. Smaller is better ($\downarrow$). \fede{Merge tables; stds; reduce significant digits}}
    \label{tab:navier-stokes-equation-quantitative-analysis}
\end{table}




% \begin{table}[]
%     \scriptsize
%     \centering
%     \begin{tabular*}{\textwidth}{c | ccccccc} 
%         \toprule
%         Time / Rollouts & GCN & GCN (MLP) & GEN & \baseline{}& \baseline +OSC(Post) & \baseline +OSC & \baseline +OSC+Adaptive \\
%         & $\times10^{-3}$ & $\times10^{-3}$ & $\times10^{-3}$ & $\times10^{-3}$ & $\times10^{-3}$ & $\times10^{-3}$ & $\times10^{-3}$ \\
%         \midrule
%         1(s) / 10 Steps & $0.5199$ & $0.4846$ & $\mathbf{0.2322}$ & $0.3731$ & $0.3820$ & $0.3802$ & $0.2678$ \\
%         2(s) / 20 Steps & $0.8876$ & $0.6710$ & $0.5291$ & $0.6020$ & $0.6891$ & $0.5682$ & $\mathbf{0.4611}$ \\
%         3(s) / 30 Steps & $2.5899$ & $2.0455$ & $1.5331$ & $1.8581$ & $1.2808$ & $0.9244$ & $\mathbf{0.8721}$ \\
%         4(s) / 40 Steps & $4.1223$ & $3.8761$ & $2.0766$ & $2.6792$ & $1.4881$ & $1.0199$ & $\mathbf{0.9622}$ \\ 
%         5(s) / 50 Steps & $6.8703$ & $5.0224$ & $2.9223$ & $3.0880$ & $1.6793$ & $1.1402$ & $\mathbf{1.0728}$ \\ 
%         \bottomrule
%     \end{tabular*}
%     \caption{TODO: for heat equation}
%     \label{tab:heat-equation-quantitative-analysis}
% \end{table}

==> tables/supplement_experiment_table.tex <==
\begin{table}[ht!]
    \centering
    \caption{Mean square error (MSE) propagation at different time stamps in seconds. Runtimes consider model inference for the full rollouts. Smaller is better ($\downarrow$). Best in \textbf{bold}; second \underline{underlined}.}
    \vspace{4mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llrccccccc}
    \toprule
    
    % Header rows
    % \multicolumn{1}{c}{Method}
    Dataset & Metric & & \multicolumn{4}{c}{Baselines} & \multicolumn{3}{c}{\ourmodel{}}
    \\
    \cmidrule(lr){4-7} \cmidrule(lr){8-10}
    & & & GCN & GNC+MLP & GEN & \baseline{} & \baseline{+OSC(Post)} & \baseline{+OSC} & \baseline{+OSC+Adaptive}  
    \\
    \midrule
    
    % Heat Equation
    \multirow{7}{*}{Ocean} & \multirow{5}{*}{MSE {\footnotesize ($\times10^{-1}$})}  
      & 1(s) & $2.23\pm0.14$ & $2.02\pm0.16$ & $\underline{1.33}\pm0.05$ & $1.45\pm0.08$ & $1.56\pm0.09$ & $1.48\pm0.07$ & $\mathbf{1.31}\pm0.10$ \\
    & & 2(s) & $2.98\pm0.21$ & $2.57\pm0.20$ & $\underline{1.65}\pm0.11$ & $2.04\pm0.12$ & $1.98\pm0.13$ & $1.87\pm0.11$ & $\mathbf{1.52}\pm0.13$ \\
    & & 3(s) & $3.55\pm0.40$ & $2.91\pm0.43$ & $2.47\pm0.21$ & $2.67\pm0.27$ & $2.55\pm0.25$ & $\underline{2.37}\pm0.20$ & $\mathbf{2.03}\pm0.28$ \\
    & & 4(s) & $4.67\pm0.97$ & $3.89\pm0.70$ & $3.37\pm0.33$ & $3.41\pm0.39$ & $3.02\pm0.37$ & $\underline{2.88}\pm0.31$ & $\mathbf{2.57}\pm0.42$ \\
    & & 5(s) & $6.02\pm1.12$ & $5.23\pm0.98$ & $4.55\pm0.52$ & $4.75\pm0.61$ & $3.82\pm0.49$ & $\underline{3.61}\pm0.38$ & $\mathbf{3.34}\pm0.44$ \\ 
    \cmidrule[0.1pt]{2-10}
    & Rollout steps \# & & 50 & 50 & 50 & 50 & 12 & 12 & 12 
    \\
    & Runtime [s] & & $3.56\pm0.15$ & $3.38\pm0.13$ & $7.11\pm0.31$ & $7.15\pm0.25$ & $1.61\pm0.12$ & $\mathbf{1.44}\pm0.09$ & $\underline{1.57}\pm0.11$ 
    \\ 
    \bottomrule
    \end{tabular}}
    \label{tab:ocean-result}
\end{table}


